Approximate k-Cover in Hypergraphs: Efficient Algorithms, and Applications

Given a weighted hypergraph $\mathcal{H}(V, \mathcal{E} \subseteq 2^V, w)$, the approximate $k$-cover problem seeks for a size-$k$ subset of $V$ that has the maximum weighted coverage by \emph{sampling only a few hyperedges} in $\mathcal{E}$. The problem has emerged from several network analysis applications including viral marketing, centrality maximization, and landmark selection. Despite many efforts, even the best approaches require $O(k n \log n)$ space complexities, thus, cannot scale to, nowadays, humongous networks without sacrificing formal guarantees. In this paper, we propose BCA, a family of algorithms for approximate $k$-cover that can find $(1-\frac{1}{e} -\epsilon)$-approximation solutions within an \emph{$O(\epsilon^{-2}n \log n)$ space}. That is a factor $k$ reduction on space comparing to the state-of-the-art approaches with the same guarantee. We further make BCA more efficient and robust on real-world instances by introducing a novel adaptive sampling scheme, termed DTA.

==> body/distributed.tex <==
\section{Distributed Hypergraph Sketching}
\label{sec:dist}
\subsection{Distributed Hypergraph Sketch (\dhs{})}
We consider a distributed environment in which there are $p$ worker machines, i.e. $M_1, M_2, \dots, M_p$, and each of them can acquire random hyperedges independently and a master machine $M_a$ that can communicate back and forth with worker machines.

The distributed sketch (\dhs{}) has the following components:

\textbf{Data}: on machine $M_i, \forall i = 1, \dots, p$, we have
\begin{itemize}
	\item $S$ - set of selected nodes, initially $S = \emptyset$,
	\item $\mathcal{E}^{(i)}$ - set of hyperedges uncovered by $S$, initially $\mathcal{E}^{(i)} = \emptyset$,
	\item $d^{(i)}_v, \forall v \in V$ - hyperdegrees of nodes in $\mathcal{E}^{(i)}$, initially $d^{(i)}_v = 0, \forall v \in V$,
	\item $d^{(i)}_S$ - coverage of set $S$, i.e. number of hyperedges covered by $S$, initially $d^{(i)}_S = 0$.
\end{itemize}

\textbf{Operators}:
\begin{itemize}
	\item \textsf{Get-Hyperedge()}: Acquire new hyperedges and update nodes' hyperdegrees.
	
	\textit{For each machine $M_2, \dots M_p$}, it keeps acquiring new hyperedges until the total size of all the hyperedges reaches to $O(\frac{n \cdot (z-d^{(i)}_S)}{k \cdot p})$. Then, they send their updates of node hyperdegrees and $d^{(i)}_S$ if they change their values due to new added hyperedges.
	
	\textit{For machine $M_1$}, it receives updates from other machines $M_2, \dots M_p$ one by one and updates its own $d^{(1)}_S$ and node hyperdegrees $d^{(1)}_v, \forall v \in V$.
	\item \textsf{Select-Node(u)}: Select node $u$ into the solution set and update the hypergraph across all the machines.
	
	\textit{For machine $M_1$}, it selects node $u$ into the maintained solution set and broadcast $u$ and updated value of $d^{(1)}_S$ to all other machines. Then, it waits for updates on hyperdegree changes due to new selection of $u$ from other machines and update $d^{(1)}_v, \forall v \in V$ accordingly.
	
	\textit{For each machine $M_2, \dots, M_p$}, it receives node selection $u$ and $d^{(1)}_S$ from machine $M_1$ and adds $u$ to $S$ as well as $d^{(i)}_S = d^{(1)}_S$. It then removes all the hyperedges that contain $u$ and hyperdegrees of nodes affected by the removals. Afterwards, it sends the hyperdegrees updates to machine $M_1$ for those nodes whose hyperdegrees are changed only.
\end{itemize}

\textbf{Communication complexity}. The communication only happens between $M_1$ and other machines and the total amount of communicating data is bounded by the total size of all the hyperedges acquired. Specifically, in \textsf{Get-Hyperedge()}, $M_1$ sends hyperdegree updates of nodes affected by adding new hyperedges, hence, only the nodes appearing in new hyperedges are updated. Similarly, in \textsf{Select-Node(u)}, only the nodes appearing in removed hyperedges need to be updated. Thus, each node in a hyperedge incurs at most 2 updates when adding and removing hyperedges.

\textbf{Implementation on MapReduce framework}. This distributed sketch can be conveniently implemented on the popular MapReduce framework. For \textsf{Get-Hyperedge()}, the reduce tasks are performed in each machine $M_2, \dots, M_p$ that acquiring new hyperedges and the map task is done in $M_1$ that gathers updates from other machines. Similarly, for \textsf{Select-Node(u)}, the map task is selecting $u$ in $M_1$ and broadcast the update to other machine while machines $M_2, \dots, M_p$ run reduce tasks which update their hyperedges and send hyperdegree updates back to $M_1$.

TODO: 
\begin{itemize}
\item Data structure for each machine (Master + Worker): $S, d_S, \mathcal E$
\item Set of Operations:
		\begin{itemize}
        	\item Get-Hyperedges: Master (how sketch is updated)/ Worker (batch size, how sketch is updated) -> more efficient than transfering the actual hyperedges
            \item Select-Node($u$): Master / Worker
        \end{itemize}
\item Bound on the communication (Given an arbitrary set of Get-Hyperedges and Select-Node, the communication is bounded by the total size of the sketch),  effect of batch-size  on communication/computational time.
\item How the operations can be implemented in Map-reduce model?
\end{itemize}





Under this model, four important factors determine the performance of a distributed algorithm: 1) communication complexity; 2) maximum load on any machine; 3) total load on all the machines and 4) number of rounds of computation. We summarize these three aspects of our algorithm against the existing ones in Table~\ref{tab:dist}.
\begin{table*}[!t]
	\caption{Summary of distributed Max-$k$-Cover algorithms.}
	\label{tab:dist}
	\centering
	\begin{tabular}{cccccc}
		\toprule
		Algorithm & Approximation & Communication & Load per machine & Total load & \#round \\
		\midrule
		DHS (here) & $1-\frac{1}{e}-\epsilon$ & $O(n \log n)$ & $O(n \log n)$ & $O(n \log n)$ & $2k$\\
		\bottomrule
	\end{tabular}
\end{table*}

\subsection{Solving Max-$k$-Cover with Distributed Hypergraph Sketch}
We develop a fast space-efficient version of \tpa{} algorithm on the distributed environment taking advantages of multiple machines to scale up the algorithm.

\textbf{Main idea.}

\begin{algorithm}
	\caption{\dtpa{} - Distributed \tpa{} algorithm}
	\label{alg:tpa_dist_2}
	Initialize a distributed sketch \dhs{} $\mathcal{H}$ on $p$ machines;\\
	\For{$i = 1 \text{ to } k$}{
		$\mathcal{H}.$\textsf{Get-Hyperedge()};\\
		$u_{\max} = \max_{v \in V \backslash S} d^{(1)}_v$;\Comment{Select on machine $M_1$}\\
		$\mathcal{H}.$\textsf{Select-Node($u_{\max}$)};\\
	}
	\If(\Comment{Run on machine $M_1$}){$\ob(S) \geq z$}{
		
	}
\end{algorithm}

\begin{algorithm}
	\caption{\dtpa{} - Distributed \tpa{} algorithm}
	\label{alg:tpa_dist}
	\KwIn{A budget $k$ and a threshold $z$ on $\OPT_k$}
	\KwOut{$T$ - max number of acquired hyperedges s.t. $z \geq opt^{(T)}_k \geq (1-1/e) z$ and a candidate solution $S$}
	\nonl \textbf{Initialize worker $M_i, i = 1,\dots,p$:} \\
	\quad $S \leftarrow \emptyset$; \Comment{selected nodes}\\
	\quad $\forall v \in V, d^{(i)}_v = 0$; \Comment{nodes' hyperdegrees}\\
	\quad $\mathcal{E}^{(i)} = \emptyset$; \Comment{hyperedges NOT covered by $S$ in $M_i$}\\
	\quad $d_{S} = 0; $\Comment{total number of hyperedges covered by $S$};\\
	\nonl \textbf{Initialize master $M_a$}:\\
	\quad $S \leftarrow \emptyset$; \Comment{selected nodes}\\
	\quad $\forall v \in V, d^{(a)}_v = 0$; \Comment{nodes' hyperdegrees}\\
	\quad $d_{S} = 0; $\Comment{total number of hyperedges covered by $S$};\\
%	$d_{S} \leftarrow 0; $\Comment{Number of hyperedges covered by $S$};\\
%	$\mathcal{E} \leftarrow \emptyset$ \Comment{Hyperedges NOT covered by $S$};\\
	
	\While{$|S| < k$}{
		\nonl \textbf{Worker $M_i, \forall i = 1,\dots,p$}: \\
		\quad Acquire hyperedges untill the total size reaches $O(\frac{n \cdot z}{k \cdot p})$ or $\max_{v \notin S} d^{(i)}_v \geq \frac{z-d_S}{k}$;\\
		\quad Send nodes' hyperdegree changes to $M_a$;\\
		\nonl \textbf{Master $M_a$}:\\
		{	
			\SetInd{1.5em}{1em}
			\quad \For{$i = 1$ \emph{\textbf{to}} $p$}{
				Receive updates from $M_i$ and update $d^{(a)}_v, \forall v \in V$;\\
				\SetInd{0.5em}{1em}
				\If{$\exists v, d^{(a)}_v \geq \frac{z - d_S}{k}$}{
					Add $u=\displaystyle\arg\max_{v \notin S} d^{(a)}_v$ to $S$ and update $d_S$;\\
					Send $u$ and $d_S$ to all the worker machines;\\
				}
			}
		}
		\nonl \textbf{Worker $M_i, \forall i = 1,\dots,p$}: \\
		{
			\SetInd{1.5em}{1em}
			\quad \If{Receive $u$ from $M_a$}{
				Update $d^{(i)}_v, \forall v \in V$ and $\mathcal{E}^{(i)}$;\\
				Send nodes' hyperdegree changes to $M_a$;\\
			}
		}
		\nonl \textbf{Master $M_a$}:\\
		{
			\SetInd{1.5em}{1em}
			\quad \For{$i = 1$ \emph{\textbf{to}} $p$}{
				Receive updates from $M_i$ and update $d^{(a)}_v, \forall v \in V$;\\
			}
		}
	}

	\If{$\ob(S) > z$}{
		Determine $M_j$ whose updates $M_a$ reveives at last;\\
		\nonl \textbf{Worker $M_j$}: \\
		{
			\quad Send hyperedges acquired in the last iteration to $M_a$;\\
		}
		\nonl \textbf{Master $M_a$}: \\
		{
			\quad Remove added nodes in $S$ due to updates from $M_j$;\\
			\quad Receive set of hyperedges from $M_j$, denoted by $\mathcal{E}$;\\
		}
		\For{$i = |S| \emph{\textbf{ to }} k$}{
			\nonl \textbf{Master $M_a$}: \\
			{
				\SetInd{1.5em}{1em} \quad \While{$|\mathcal{E}| > 0$ and $\forall v, d^{(a)}_v < \frac{z - d_S}{k}$}{
					Get a hyperedge in $\mathcal{E}$ and add to $\mathcal{E}^{(a)}$;\\
					Update $d_S$ and $d^{(a)}_v, \forall v \in V$.
				}
			}
			\SetInd{1.5em}{1em}
			\quad \ForEach{hyperedge $E_j$ received from $M_j$}{
				\SetInd{0.5em}{1em}
				\If{$\exists v, d^{(a)}_v \geq \frac{z - d_S}{k}$}{
					Add $u=\displaystyle\arg\max_{v \notin S} d^{(a)}_v$ to $S$;\\
					
					Send $u$ to all the worker machines;\\
				}
			}
		}
	}
	\textbf{return} <$T=\#\text{hyperedges acquired}, S$>;\\
\end{algorithm}


\subsection{Analysis}

==> body/exp.tex <==
%\begin{figure*}[!ht]
%	\subfloat[Epinions]{
%		\includegraphics[width=0.24\linewidth]{figures/epinions_IC_trivalency_time}
%		%		\label{fig:hep_lt_inf}
%	}
%	\subfloat[Orkut]{
%		\includegraphics[width=0.24\linewidth]{figures/orkut_IC_trivalency_time}
%		%		\label{fig:phy_lt_inf}
%	}
%	\subfloat[Twitter]{
%		\includegraphics[width=0.24\linewidth]{figures/twitter_IC_trivalency_time}
%		%		\label{fig:dblp_lt_inf}
%	}
%	\subfloat[Friendster]{
%		\includegraphics[width=0.24\linewidth]{figures/friendster_IC_trivalency_time}
%		%		\label{fig:twitter_lt_inf}
%	}
%	\vspace{-0.15in}
%	\caption{Running time on the \ic{} diffusion model and \textsf{TRI} edge weight model.}
%	\label{fig:time_ic_tri}
%	\vspace{-0.3in}
%\end{figure*}
%\begin{figure*}[!ht]
%	\subfloat[Epinions]{
%		\includegraphics[width=0.24\linewidth]{figures/epinions_IC_trivalency_mem}
%		%		\label{fig:hep_lt_inf}
%	}
%	\subfloat[Orkut]{
%		\includegraphics[width=0.24\linewidth]{figures/orkut_IC_trivalency_mem}
%		%		\label{fig:phy_lt_inf}
%	}
%	\subfloat[Twitter]{
%		\includegraphics[width=0.24\linewidth]{figures/twitter_IC_trivalency_mem}
%		%		\label{fig:dblp_lt_inf}
%	}
%	\subfloat[Friendster]{
%		\includegraphics[width=0.24\linewidth]{figures/friendster_IC_trivalency_mem}
%		%		\label{fig:twitter_lt_inf}
%	}
%	\vspace{-0.15in}
%	\caption{Memory usage on the \ic{} diffusion model and \textsf{TRI} edge weight model.}
%	\label{fig:mem_ic_tri}
%	\vspace{-0.15in}
%\end{figure*}

%\begin{figure}[!ht]
%	\vspace{-0.1in}
%	\subfloat[On \textsf{WC} model]{
%		\includegraphics[width=0.49\linewidth]{figures/upperbound_wc}
%		%		\label{fig:hep_lt_inf}
%	}
%	\subfloat[On \textsf{TRI} model]{
%		\includegraphics[width=0.49\linewidth]{figures/upperbound_tri}
%		%		\label{fig:phy_lt_inf}
%	}
%	\vspace{-0.15in}
%	\caption{Influence and time relative ratios between the Requirement and Top-$k$ upper bound functions.}
%	\label{fig:bounds} 
%	\vspace{-0.15in}
%\end{figure}
\begin{table*}\scriptsize
	\centering
	\caption{Measure \dta{} on different problems for $k = 100$ and $\epsilon = 0.05$ (measured in second (or h for hour)).}
	\vspace{-0.1in}
	\begin{tabular}{l r r r rr rr rr}
		\toprule
		& & & & \multicolumn{2}{c}{Sketch Size} & \multicolumn{2}{c}{Running Time} &
		\multicolumn{2}{c}{Quality}\\
		\cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10}
		\textbf{Problems} &\textbf{Data} & \#nodes & \#edges & \dta{} & \fs{}& \dta{} & \fs{} & \dta{} & \fs{}\\
		\midrule
 		Dominating Set& DBLP & 655K & 2M & \textbf{1.3M} & 3.7M &\textbf{2.6} & 3.1 &{0.22} & {0.22}\\
		 & Orkut & 3M & 234M &\textbf{15M} & 1.14B & \textbf{47} &1048 & 0.87 &{0.89}\\
		 & Twiter & 41.7M & 1.5B & \textbf{3.3M} & \textbf{474M} &\textbf{27} &457 & 0.73 & {0.74}\\
		 \midrule
		 Influence Maximiation & DBLP & 655K & 2M & \textbf{3.4M} & 9.5M &18.7 &{\textbf{16}} & 0.0031 & {0.0032}\\
		 & Orkut & 3M & 234M &\textbf{20.8M} &858M &\textbf{1652} &1723 & 0.69 & 0.68\\
		 & Twiter & 41.7M & 1.5B &\textbf{171M} &3.8B &9614 & \textbf{9573} &0.24 & 0.25\\
		 \midrule
		 Lanmark Selection& DBLP & 655K & 2M &\textbf{65k} &245k &\textbf{78} & 90 &0.22 & 0.22\\
		 & Orkut & 3M & 234M &\textbf{31K} &268K &110 & \textbf{108} &0.62 &0.67\\
		 & Twiter & 41.7M & 1.5B &\textbf{422K} &3.6M &\textbf{1216} &1438 &0.58 &0.60\\
		 \midrule
		 K-path & DBLP & 655K & 2M &\textbf{178k} &466k &\textbf{1} &\textbf{1} &0.14 &0.15\\
		 & Orkut & 3M & 234M & \textbf{2M} &4.2M &22 &\textbf{21} &0.05 & 0.05\\
		 & Twiter & 41.7M & 1.5B &\textbf{58k} &137k &16 &\textbf{14} &0.36 &0.36\\
		\bottomrule
	\end{tabular}
	\label{tab:rtime}
	\vspace{-0.1in}
\end{table*}
\setlength\tabcolsep{2pt}
\begin{table*}\scriptsize
	\centering
	\caption{Running time of different algorithms for $k = 100$ and $\epsilon = 0.1$ (measured in second (or h for hour)).}
	\vspace{-0.1in}
	\begin{tabular}{l r r rrrrrr rrrrr rrrr rrr}
		\toprule
		& & & \multicolumn{6}{c}{\textbf{Betweenness}} & \multicolumn{5}{c}{\textbf{Coverage}} & \multicolumn{4}{c}{\textbf{Motif-based}} & \multicolumn{3}{c}{\textbf{$K$-Path}} \\
		\cmidrule(lr){4-9} \cmidrule(lr){10-14} \cmidrule(lr){15-18} \cmidrule(l){19-21}
		\textbf{Data} & \#nodes & \#edges & \textsf{EXH.} & \hedge{} & \yalg{} & \IMM$_b$ & \SSA$_b$ & \dta{} & \textsf{EXH.} & \yalg{} & \IMM$_c$ & \SSA$_c$ & \dta{} & \textsf{EXH.} & \IMM$_t$ & \SSA$_t$ & \dta{} & \IMM$_k$ & \SSA$_k$ & \dta{} \\
		\midrule
		Ego-Facebook & 4\textsf{K} & 88\textsf{K} & 246.7 & 10.4 & 9.1 & 13.6 & 0.8 & \textbf{0.0} & 525.1 & 2.4 & 17.9 & 1.1 & \textbf{0.0} & 0.1 & 0.4 & 0.0 & \textbf{0.0} &  0.6 & 0.1 & \textbf{0.0} \\
		CA-GrQc & 5\textsf{K} & 14\textsf{K} & 882.6 & 6.5 & 3.0 & 4.5 & 0.3 & \textbf{0.0} & 670.8 & 1.0 & 5.0 & 0.3 & \textbf{0.0} & \textbf{0.0} & 0.2 & 0.0 & \textbf{0.0} &  0.9 & 0.1 & \textbf{0.0} \\
		CA-HepTh & 10\textsf{K} & 26\textsf{K} & 882.6 & 13.4 & 7.2 & 8.6 & 0.8 & \textbf{0.1} & 0.9h & 2.7 & 8.8 & 0.5 & \textbf{0.1} & \textbf{0.0} & 1.0 & 0.1 & \textbf{0.0} &  1.2 & 0.2 & \textbf{0.0} \\
		Email-Enron & 37\textsf{K} & 184\textsf{K} & 3.8h & 106.7 & 62.9 & 27.6 & 1.3 & \textbf{0.1} & 14.8h & 16.5 & 21.9 & 2.1 & \textbf{0.1} & 0.2 & 3.7 & 0.3 & \textbf{0.0} &  0.4 & \textbf{0.1} & \textbf{0.1} \\
		loc-Brightkite & 58\textsf{K} & 214\textsf{K} & \textsf{dnf} & 212.4 & 82.6 & 40.5 & 1.7 & \textbf{0.3} & \textsf{dnf} & 29.7 & 44.8 & 2.1 & \textbf{0.1} & \textbf{0.1} & 2.7 & 0.2 & \textbf{0.1} &  2.0 & \textbf{0.1} & \textbf{0.1} \\
		soc-Epinions1 & 76\textsf{K} & 509\textsf{K} & \textsf{dnf} & 383.9 & 192.8 & 55.8 & 7.7 & \textbf{0.6} & \textsf{dnf} & 51.0 & 73.8 & 4.5 & \textbf{0.2} & 0.2 & 6.2 & 0.4 & \textbf{0.1} &  1.7 & \textbf{0.1} & \textbf{0.1} \\
		\bottomrule
	\end{tabular}
	\label{tab:rtime}
	\vspace{-0.1in}
\end{table*}

%\renewcommand{\arraystretch}{1}
%\setlength\tabcolsep{1.5pt}
%\begin{table*}[!h] \scriptsize
%	\centering
%	%\vspace{-0.05in}
%	\caption{Performance on the Betweenness Centrality Maximization (\BCM{}) problem for $k=100$ and $\epsilon = 0.1$ (for \dta{}, \IMM{} and \DPIMA{}) (\textsf{EXH.} denotes \exhaust{}, \textsf{dnf}: ``did not finish" within 12h, \textsf{mem}: ``out of memory").}
%	\vspace{-0.1in}
%	\begin{tabularx}{\textwidth}{l rr *{18}{Y}}
%		\toprule
%		& & & \multicolumn{6}{c}{\textbf{Running Time [s (or h)]}} & \multicolumn{6}{c}{\textbf{Total Memory [M (or G)]}} &  \multicolumn{6}{c}{\textbf{Betweenness Centrality}}
%		%		 & \multicolumn{3}{c}{\textbf{\#Samples }} 
%		\\
%		\cmidrule(lr){4-9}  \cmidrule(lr){10-15} \cmidrule(lr){16-21} 
%		%		\cmidrule(lr){16-18} 
%		\textbf{Data} & \textbf{\#Nodes}& \textbf{\#Edges} & \textsf{EXH.} & \hedge{} & \yalg{} & \IMM{} & \DPIMA{} & \dta{}  & \textsf{EXH.} & \hedge{} & \yalg{} & \IMM{} & \DPIMA{} & \dta{}  & \textsf{EXH.} & \hedge{} & \yalg{} & \IMM{} & \DPIMA{} & \dta{}  
%		%		& \hedge{} & \yalg{} & \dta{} 
%		\\
%		\midrule
%		Ego-Facebook & 4\textsf{K} & 88\textsf{K} & 246.7 & 10.4 & 9.1 & 13.6 & 0.8 & \textbf{0.0} & 13.5 & 15.4 & 17.6 & 23.6 & 19.7 & \textbf{8.1} & 0.96 & 0.96 & 0.96 & 0.95 & 0.95 & 0.92 
%		%		& 205 & 205 & 422 
%		\\
%		CA-GrQc & 5\textsf{K} & 14\textsf{K} & 882.6 & 6.5 & 3.0 & 4.5 & 0.3 & \textbf{0.0} & 12.7 & 13.9 & 16.3 & 23.3 & 18.6 & \textbf{6.6} & 0.55 & 0.56 & 0.57 & 0.55 & 0.57 & 0.50
%		%		 & 212 & 212 & 995 
%		\\
%		CA-HepTh & 10\textsf{K} & 26\textsf{K} & 882.6 & 13.4 & 7.2 & 8.6 & 0.8 & \textbf{0.1} & 13.1 & 15.1 & 17.9 & 30.2 & 20.4 & \textbf{8.2} & 0.55 & 0.53 & 0.53 & 0.53 & 0.54 & 0.51
%		%		& 227 & 227 & 1330 
%		\\
%		Email-Enron & 37\textsf{K} & 184\textsf{K} & 3.8h & 106.7 & 62.9 & 27.6 & 1.3 & \textbf{0.1} & \textbf{16.2} & 21.2 & 26.9 & 40.3 & 26.1 & 18.4 & 0.76 & 0.76 & 0.76 & 0.75 & 0.76 & 0.67
%		%		& 258 & 258 & 876 
%		\\
%		loc-Brightkite & 58\textsf{K} & 214\textsf{K} & \textsf{dnf} & 212.4 & 82.6 & 40.5 & 1.7 & \textbf{0.3} & \textsf{dnf} & 28.2 & 29.2 & 45.9 & 29.0 & \textbf{23.6} & \textsf{dnf} & 0.74 & 0.73 & 0.73 & 0.73 & 0.70
%		%		& 269 & 269 & 841
%		\\
%		soc-Epinions1 & 76\textsf{K} & 509\textsf{K} & \textsf{dnf} & 383.9 & 192.8 & 55.8 & 7.7 & \textbf{0.6} & \textsf{dnf} & 33.6 & 36.0 & 57.4 & 33.6 & \textbf{29.4} & \textsf{dnf} & 0.66 & 0.66 & 0.66 & 0.65 & 0.63 
%		%		& 276 & 276 & 958
%		\\
%		\bottomrule    		
%	\end{tabularx}
%	\label{tab:compare_bcm}
%	\vspace{-0.1in}
%\end{table*}
%\setlength\tabcolsep{3pt}
%\begin{table}[!h] \small
%	\centering
%	\caption{Running times on \CCM{}, \TCM{} and \PCM{} for $k=100$. }
%	\vspace{-0.15in}
%	\begin{tabular}{l rrr r rr r r}
%		\toprule
%		& \multicolumn{3}{c}{\textbf{\CCM}} && \multicolumn{2}{c}{\bf \TCM{}} && \multicolumn{1}{c}{\textbf{\PCM}} \\
%		\cmidrule{2-4} \cmidrule{6-7} \cmidrule{9-9}
%		\textbf{Data} & \exhaust{} & \yalg{} & \dta{}  && \exhaust{} & \dta{}  && \dta{} \\
%		\midrule			
%		%		Ego-F. & 525.1 & 0.1 & \textbf{0.0} && 13.5 & 14.5 & \textbf{5.0} && 0.99 & 0.97 & 0.94 \\
%		%		CA-G. & 670.8 & \textbf{0.0} & \textbf{0.0} && 12.7 & 13.1 & \textbf{3.2} && 0.60 & 0.39 & 0.50\\
%		%		CA-H. & 0.9h & 0.1 & \textbf{0.0} && 13.4 & 13.4 & \textbf{4.30} && 0.65 & 0.39 & 0.50 \\
%		%		Email & 14.8h & 0.6 & \textbf{0.1} && 17.0 & 18.6 & \textbf{13.6} && 0.82 & 0.65 & 0.70 \\
%		%		loc-B. & \textsf{dnf} & 1.2 & \textbf{0.1} &&\textsf{dnf}& 20.4 & \textbf{18.4} &&\textsf{dnf}& 0.74 &0.76 \\
%		%		soc-E. & \textsf{dnf} & 2.1 & \textbf{0.2} &&\textsf{dnf}& \textbf{22.7} & 24.1 &&\textsf{dnf}& 0.72 & 0.76\\
%		%		Ego-Facebook & 525.1 & 0.1 & \textbf{0.0} && 0.1 & \textbf{0.0} && 0.0 \\
%		CA-GrQc & 670.8 & \textbf{0.0} & \textbf{0.0} && \textbf{0.0} & \textbf{0.0} && 0.0\\
%		CA-HepTh & 0.9h & 0.1 & \textbf{0.0} &&  \textbf{0.0}& \textbf{0.0}  && 0.0 \\
%		Email-Enron & 14.8h & 0.6 & \textbf{0.1} && 0.2 & \textbf{0.0} && 0.0 \\
%		loc-Brightkite & \textsf{dnf} & 1.2 & \textbf{0.1} && 0.1 &  \textbf{0.0} && 0.0 \\
%		soc-Epinions1 & \textsf{dnf} & 2.1 & \textbf{0.2} && 0.2 &  \textbf{0.0} && 0.0\\
%		\bottomrule    		
%	\end{tabular}
%	\label{tab:compare_ccm}
%\end{table}
%\setlength\tabcolsep{6pt}
%\begin{table*}[!h] \scriptsize
%	\centering
%	\caption{Performance on Coverage Centrality Maximization (\CCM{}) for $k=100$ and $\epsilon = 0.1$ (for \dta{}, \IMM{} and \DPIMA{}).}
%	\vspace{-0.1in}
%	\begin{tabular}{l rrrrr r rrrrr r rrrrr}
%		\toprule
%		& \multicolumn{5}{c}{\textbf{Running Time [s (or h)]}} && \multicolumn{5}{c}{\textbf{Total Memory [M (or G)]}} && \multicolumn{5}{c}{\textbf{Coverage Centrality}}
%		%		 && \multicolumn{2}{c}{\textbf{\#Samples }} 
%		\\
%		\cmidrule{2-6}  \cmidrule{8-12} \cmidrule{14-18} 
%		%		\cmidrule{14-15} 
%		\textbf{Data} & \textsf{EXH.} & \yalg{} & \IMM{} & \DPIMA{} & \dta{}  && \textsf{EXH.} & \yalg{} & \IMM{} & \DPIMA{} & \dta{}  && \textsf{EXH.} & \yalg{} & \IMM{} & \DPIMA{} & \dta{}  
%		%		&& \yalg{} & \dta{} 
%		\\
%		\midrule			
%		Ego-Facebook & 525.1 & 2.4 & 17.9 & 1.1 & \textbf{0.0} & & 13.5 & 15.2 & 28.4 & 20.0 & \textbf{8.0} && 0.99 & 0.99 & 0.99 & 0.98 & 0.97 
%		%		&& 205 & 498 
%		\\
%		CA-GrQc & 670.8 & 1.0 & 5.0 & 0.3 & \textbf{0.0} && 12.7 & 13.6 & 28.9 & 19.0 & \textbf{6.8} && 0.60 & 0.59 & 0.58 & 0.59 & 0.53 
%		%		&& 212 & 919 
%		\\
%		CA-HepTh & 0.9h & 2.7 & 8.8 & 0.5 & \textbf{0.1} && 13.4 & 14.2 & 34.3 & 20.1 & \textbf{8.2} && 0.65 & 0.63 & 0.62 & 0.64 & 0.55
%		%		&& 227 & 872 
%		\\
%		Email-Enron & 14.8h & 16.5 & 21.9 & 2.1 & \textbf{0.1} && \textbf{17.0} & 20.1 & 66.3 & 28.3 & 18.3 && 0.82 & 0.81 & 0.79 & 0.80 & 0.70 
%		%		&& 258 & 824 
%		\\
%		loc-Brightkite & \textsf{dnf} & 29.7 & 44.8 & 2.1 & \textbf{0.1} &&\textsf{dnf}& 22.0 & 65.6 & 31.2 & 23.6 &&\textsf{dnf} & 0.86 & 0.86 & 0.86 & 0.77
%		%		&& 269 & 777 
%		\\
%		soc-Epinions1 & \textsf{dnf} & 51.0 & 73.8 & 4.5 & \textbf{0.2} && \textsf{dnf} & \textbf{24.9} & 90.2 & 33.2 & 29.4 && \textsf{dnf} & 0.88 & 0.88 & 0.85 & 0.74 
%		%		&& 276 & 789
%		\\
%		\bottomrule
%	\end{tabular}
%	\label{tab:compare_ccm}
%	\vspace{-0.1in}
%\end{table*}
%
%\setlength\tabcolsep{3.4pt}
%\begin{table*}[!h] \scriptsize
%	\centering
%	\caption{Performance on Triangle and $K$-Path Centrality Maximizations for $k=100$ and $\epsilon = 0.1$ (for \dta{}, \IMM{} and \DPIMA{}).}
%	\vspace{-0.1in}
%	\begin{tabular}{l rrrr rrrr rrrr rrrr rrrr rrrr}
%		\toprule
%		& \multicolumn{12}{c}{\textbf{Triangle Centrality Maximization}} & \multicolumn{12}{c}{\textbf{$K$-Path Centrality Maximization}} \\
%		\cmidrule(lr){2-13} \cmidrule(lr){14-25}
%		& \multicolumn{4}{c}{\textbf{Running Time [s (or h)]}} & \multicolumn{4}{c}{\textbf{Total Memory [M (or G)]}} & \multicolumn{4}{c}{\textbf{Triangle Centrality}} & \multicolumn{4}{c}{\textbf{Running Time [s (or h)]}} & \multicolumn{4}{c}{\textbf{Total Memory [M (or G)]}} & \multicolumn{4}{c}{\textbf{$K$-Path Centrality}} \\
%		\cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13} \cmidrule(lr){14-17} \cmidrule(lr){18-21} \cmidrule(lr){22-25}
%		\textbf{Data} & \textsf{EXH.} & \IMM{} & \DPIMA{} & \dta{} & \textsf{EXH.} & \IMM{} & \DPIMA{} & \dta{} & \textsf{EXH.} & \IMM{} & \DPIMA{} & \dta{}  & \textsf{EXH.} & \IMM{} & \DPIMA{} & \dta{} & \textsf{EXH.} & \IMM{} & \DPIMA{} & \dta{} & \textsf{EXH.} & \IMM{} & \DPIMA{} & \dta{} \\
%		\midrule			
%		Ego-Facebook & 0.1 & 0.4 & 0.0 & \textbf{0.0} & 15.5 & 28.9 & 20.2 & \textbf{9.1} & 0.26 & 0.20 & 0.18 & 0.21 & 0.1 & 0.6 & 0.1 & \textbf{0.0} & 15.5 & 48.6 & 30.5 & \textbf{9.0} & 0.18 & 0.18 & 1.18 & 0.17 \\
%		CA-GrQc & \textbf{0.0} & 0.2 & 0.0 & \textbf{0.0} & 13.3 & 23.0 & 19.0 & \textbf{8.5} & 0.75 & 0.67 & 0.65 & 0.63 & \textbf{0.0} & 0.9 & 0.1 & \textbf{0.0} & 13.3 & 73.2 & 29.4 & \textbf{6.4} & 0.13 & 0.13 & 0.12 & 0.12 \\
%		CA-HepTh & \textbf{0.0} & 1.0 & 0.1 & \textbf{0.0} & 14.1 & 32.6 & 21.6 & \textbf{10.8} & 0.35 & 0.33 & 0.31 & 0.29 & \textbf{0.0} & 1.2 & 0.2 & \textbf{0.0} & 14.1 & 122.8 & 42.7 & \textbf{8.5} & 0.07 & 0.07 & 0.07 & 0.07 \\
%		Email-Enron & 0.2 & 3.7 & 0.3 & \textbf{0.0} & 22.3 & 43.1 & 26.3 & \textbf{17.2} & 0.39 & 0.37 & 0.38 & 0.34 & 0.2 & 0.4 & 0.1 & \textbf{0.1} & 22.3 & 57.9 & 28.1 & \textbf{16.4} & 0.30 & 0.30 & 0.30 & 0.29 \\
%		loc-Brightkite & \textbf{0.1} & 2.7 & 0.2 & \textbf{0.1} & 25.3 & 46.7 & 29.5 & \textbf{23.6} & 0.28 & 0.26 & 0.23 & 0.23 & \textbf{0.1} & 2.0 & 0.1 & \textbf{0.1} & 25.3 & 160.3 & 41.6 & \textbf{20.7} & 0.07 & 0.07 & 0.07 & 0.07 \\
%		soc-Epinions1 & 0.2 & 6.2 & 0.4 & \textbf{0.1} & 29.1 & 57.2 & 31.7 & \textbf{28} & 0.27 & 0.26 & 0.27 & 0.27 & 0.2 & 1.7 & 0.1 & \textbf{0.1} & 29.1 & 142.1 & 44.0 & \textbf{24.1} & 0.11 & 0.11 & 0.08 & 0.07 \\
%		\bottomrule
%	\end{tabular}
%	\label{tab:compare_motif-based}
%	\vspace{-0.1in}
%\end{table*}

%\vspace{-0.1in}
\section{Experiments}
\label{sec:exps}
We experimentally test our algorithms\footnote{For reproducibility, we will make the source code public.} against the state-of-the-art methods on different applications. The results show a significant saving in terms of running time and memory consumption provided by our algorithm compared to the others. This demonstrates our advantages of having small time and space complexities. Comparison between \dta{} and \tpa{} shows that \dta{} uses in orders of magnitude smaller time and memory than \tpa{} proving the effectiveness of our accurate quality assessment deployed in \dta{}.

\vspace{0.03in}

\noindent \textbf{Algorithms.}
On centrality max, we compare \dta{} with:
\begin{itemize}
	\item \hedge{} \cite{Mahmoody16} and \yalg{} \cite{Yoshida14}: state-of-the-art algorithms for centrality maximizations that provide theoretical guarantees but resort to heuristic setting of $\frac{2 \log(2n^3)}{\epsilon^2}$ samples for practical uses. We set $\epsilon = 0.1$.
	\vspace{-0.02in}
	\item \exhaust{} greedy which implements the greedy algorithm using the exact computation of centrality.
	\item Adaptations of \IMM{} \cite{Tang15} and \DPIMA{} \cite{Nguyen163} to centrality maximizations. The extensions are straightforward by replacing the sampling procedure and keep all the other settings to provide the $(1-1/e-\epsilon)$ approximation ratio with probability $1-\delta$ where $\epsilon = 0.1, \delta = 1/n$. We call \IMM$_b$, \IMM$_c$, \IMM$_t$, \IMM$_k$ for adaptations of \IMM{} to betweenness, coverage, motif-based and $K$-Path centralities. Similarly for \DPIMA{} adaptations, we have \SSA$_b$, \SSA$_c$, \SSA$_t$, \SSA$_k$.
\end{itemize}

On Influence Maximization, \dta{} is compared with:
\begin{itemize}
	%	\item \DPIMA{} \cite{Nguyen163}: The current fastest \RIS{}-based algorithm with $(1-1/e-\epsilon)$-approximation guarantee.
	\item \IMM{} \cite{Tang15}, \DPIMA{} \cite{Nguyen163}: A \RIS{}-based algorithm providing $(1-1/e-\epsilon)$ approximation guarantee with prob. $1-\delta$. Again, we use the common setting of $\epsilon = 0.1, \delta = 1/n$. \DPIMA{} originally contains errors \cite{Huang17} but fixed in \cite{dssa_fix}.
	\item \PMC{} \cite{Ohsaka14}: A Monte-Carlo simulation pruned method with no guarantee. We use the default $200$ DAGs.
	\item \textsf{TipTop} \cite{Li172}: A recent method using stochastic programming to achieve $(1-\epsilon)$-approximation ratio. To be compatible, we set $\epsilon = 1/e+0.1, \delta = 1/n$.
\end{itemize}
%Specifically, \exhaust{} iteratively selects nodes that maximize the marginal centrality with respect to the selected nodes. Here, the marginal centrality of a node $u$ with respect to a set $S$ is defined as 
%\begin{align}
%	\Delta(u,S) = \textsf{C}(S \cup \{u\}) - \textsf{C}(S),
%\end{align}
%where $\textsf{C}(S)$ denotes the centrality of set $S$. 
%Although \hedge{} \cite{Mahmoody16} and \yalg{} \cite{Yoshida14} provides theoretical approximation guarantee, their settings to achieve it are too conservative and they resort to heuristic approach of selecting a smaller number, i.e. $\frac{2 \log(2n^3)}{\epsilon^2}$, of samples as default in their implementations. Note that  unlike their approach, \dta{} provides rigorous guarantees of $(1-1/e-\epsilon)$-approximate solution. We also extend the \IMM{} \cite{Tang15} and \DPIMA{} \cite{Nguyen163}, i.e. most recent approaches for \IM{}, to centrality maximizations.

We obtain the implementations of all algorithms by the authors. \DPIMA{} is the latest version after being fixed \cite{dssa_fix}. In comparison with other algorithms, \dta{} uses the requirement function and later, we study different upper-bound functions and their effects to the performance of \tpa{}/\dta{}.

%\textbf{\dta{} upper-bound functions.} We have pointed out 6 different functions that \dta{} can use, we carry tests on three of them: requirement, $\topk$ and \textsf{DF-2D}, in comparison with other state-of-the-arts and compare the quality of all 6 upper-bound functions at the end. We denote the three versions as \dta-\textsf{req}, \dta{}-{\top} and \dta{}-{2d}.

\vspace{0.03in}

\noindent \textbf{Datasets.}
On Centrality Maximization problems, we use 5 common small to moderate-size datasets \cite{Mahmoody16,Yoshida14} (summarized in Table~\ref{tab:rtime}) since the \exhaust{} algorithm cannot run on larger networks. For \IM{}, 6 real-world datasets (Table~\ref{tab:compare_im}) from \cite{snap,Kwak10} with sizes from thousands to 3.6 billion edges.

%\vspace{-0.05in}
\vspace{0.03in}

\noindent \textbf{Experimental Environment.}
All the experiments are run on a cluster of 16 Linux machines, each of which has a 2.30Ghz Intel(R) Xeon(R) CPU E5-2650 v3 40 core processor and 256GB of RAM. We limit the running time of each algorithm to be within 12 hours and memory to 100GB.

%\setlength\tabcolsep{4pt}
%\begin{table}[!htb]
%	%	\vspace{-0.1in}
%	\caption{Compare upper-bound functions}
%	\vspace{-0.1in}
%	\label{tab:ubounds}
%	\centering
%	\begin{tabular}{ l  r  r  r r r }
%		\toprule	
%		\textbf{Data} & \bf \textsf{Req.} & \bf \textsf{Top-$k$} & \bf\textsf{Dual-1} & \bf\textsf{Dual-2} & \bf LP\\
%		\midrule
%		PHY & 7266 & 7002 & 6400 & 4642 & 4504 \\
%		Epinions & 1816 & 1816 & 1600 & 1583 & 1518\\
%		DBLP & 7434 & 7103 & 6400 & 4591 & 4539\\
%		Orkut & 498 & 446 & 400 & 400 & 400 \\
%		Twitter & 299& 299 & 200 & 200 & \textsf{dnf} \\
%		Friendster & 100 & 100 & 100 & 100 & \textsf{dnf}\\
%		\bottomrule
%	\end{tabular}
%	%	\vspace{-0.1in}
%\end{table}

\subsection{Full Sketch vs. Reduced sketch}
\label{subsec:effectinvess}
We show that our reduced sketch $\E_r$ saves a huge amount of memory compared to the full sketch while keeping the time and solution quality comparable.

We first run \dta{} with the basic requirement function and $\epsilon = 0.1, \delta = 1/n$ and obtain the peak total size of the reduced and full sketch. Here, we also maintain the full sketch $\E_f$ to run the greedy algorithm \cite{Nemhauser81} on $\E_f$ to find the solution on the same set of sampled hyperedges. This provides peak sketch size and solution quality of using reduced and full sketches. To get the running time, we take the last trial threshold $z$ in \dta{} and run \tpa{} with that $z$. We simulate the sampling of the same number of hyperedges $T$ returned by \tpa{} to get the running time for full sketch.

The results on two applications of Landmark Selection, aka \CCM{}, and Influence Maximization (\textsf{TRI} edge model and \ic{} diffusion model) on 4 relatively large networks (Table~\ref{tab:compare_im}) are shown in Figure~\ref{fig:mem_time_quality}. It shows that the reduced sketch is very space-efficient compared to the full version, e.g., commonly uses $<$ 10\% of space for the full sketch. There are cases, e.g., \IM{} on PHY and DBLP, that the reduced sketch is less efficient. A close look into this case reveals that these networks are sparse resulting in tiny \RIS{} hyperedges and hence, space saving of removing covered hyperedges is less. This shows that reduced sketch becomes efficient when hyperedges are large or there exists a high coverage solution.

\setlength\tabcolsep{3.5pt}
\begin{table}\small
	\centering
	\caption{Relative memory of different algorithms to \dta{}.}
	\vspace{-0.1in}
	\begin{tabular}{l rrrrrr}
		\toprule
		\textbf{Problem} & \textsf{EXHAUST} & \hedge{} & \yalg{} & \IMM$_b$ & \SSA$_b$ & \dta{} \\
		\midrule
		\BCM{} & 1.5 & 1.6 & 1.8 & 2.7 & 1.9 & 1\\
		\CCM{} & 1.5 & \_ & 1.4 & 3.6 & 2.0 & 1\\
		\TCM{} & 1.3 & \_ & \_ & 2.6 & 1.7 & 1\\
		\PCM{} & \_ & \_ & \_ & 8.1 & 3.1 & 1\\
		\bottomrule
	\end{tabular}
	\label{tab:mem_relative}
	\vspace{-0.1in}
\end{table}
\setlength\tabcolsep{3.5pt}
\begin{table}\small
	\centering
	\caption{Relative quality of different algorithms to \dta{}.}
	\vspace{-0.1in}
	\begin{tabular}{l rrrrrr}
		\toprule
		\textbf{Problem} & \textsf{EXHAUST} & \hedge{} & \yalg{} & \IMM$_b$ & \SSA$_b$ & \dta{} \\
		\midrule
		\BCM{} & 1.09 & 1.07 & 1.07 & 1.06 & 1.07 & 1 \\
		\CCM{} & 1.13 & \_ & 1.12 & 1.11 & 1.12 & 1\\
		\TCM{} & 1.16 & \_ & \_ & 1.05 & 1.00 & 1 \\
		\PCM{} & \_ & \_ & \_ & 1.11 & 1.04 & 1 \\
		\bottomrule
	\end{tabular}
	\label{tab:qual_relative}
\end{table}

\subsection{Results on Centrality Maximizations}
\textbf{Results Overview.} Our experimental evaluations are presented in Tables~\ref{tab:rtime}, \ref{tab:mem_relative} and \ref{tab:qual_relative}. Our results evidently show that \dta{} algorithm generally uses 10x less time, several time less memory while obtaining the same level of solution quality with existing state-of-the-art algorithms. Results on the \#samples are presented in our appendix.

\renewcommand{\arraystretch}{0.9}
\setlength\tabcolsep{3pt}
\begin{table*}[!ht] \scriptsize
	\centering
	\vspace{-0.05in}
	\caption{Performance of \IM{} algorithms with $k=100$ on the \ic{} diffusion model and edge weight models: \textsf{TRI} and \textsf{WC}.}
	\vspace{-0.1in}
	\begin{tabularx}{\textwidth}{c cl r r rrrrrrrrrrrrrrr}
		\toprule
		& & & & & \multicolumn{5}{c}{\textbf{Time [s (or h for hour)]}} & \multicolumn{5}{c}{\textbf{Memory [MB (or G for GB)]}} & \multicolumn{5}{c}{\textbf{Influence Spread (\% of nodes)}} 
		%		& \multicolumn{2}{c}{\textbf{\#Samples [$\times 10^3$] }} 
		\\
		\cmidrule(lr){6-10} \cmidrule(lr){11-15} \cmidrule(l){16-20} 
		%		\cmidrule(lr){14-15}
		& & \textbf{Data} & \textbf{\#Nodes}& \textbf{\#Edges} & \textsf{PMC} & \textsf{TipTop} & \IMM{} & \DPIMA{} & \dta{} & \textsf{PMC} & \textsf{TipTop} & \IMM{} & \DPIMA{} & \dta{} & \textsf{PMC} & \textsf{TipTop} & \IMM{} & \DPIMA{} & \dta{} 
		%		& \textsf{IMM} & \dta{} 
		\\
		\midrule
		\multirow{6}{*}{\textsf{TRI}} &
		\multirow{3}{*}{\textsf{Small}}
		& PHY & 37\textsf{K} & 181\textsf{K} & 5.5 & 1.8 & 7.7 & 1.2 & \textbf{0.9} & 251 & 412 & 475 & 125 & \textbf{21} & 0.011 & 0.018 & 0.018 & 0.018 & 0.017
		%		& 370.1 & \textbf{30.4}
		\\
		& & Epinions & 132\textsf{K} & 841\textsf{K} & 20.3 & 33.0 & 0.3h & 151.0 & \textbf{5.9} & 502 & 811 & 9G & 1G & \textbf{27} & 0.060 & 0.055 & 0.060 & 0.058 & 0.056
		%		& 123.0 & \textbf{2.7} 
		\\
		& & DBLP & 655\textsf{K} & 2\textsf{M} & 68.9 & 10.2 & 73.3 & 6.8 & \textbf{3.4} & 4G & 4G & 579 & 1G & \textbf{285} & 0.003 & 0.003 & 0.003 & 0.003 & 0.003
		%		& 3171.0 & \textbf{172.2}
		\\
		\cmidrule{3-20}
		& \multirow{3}{*}{\textsf{Large}}
		& Orkut & 3\textsf{M} & 234\textsf{M} & 0.8h & 3.5h & \textsf{dnf} & \textsf{dnf} & \textbf{0.6h} & 21G & 89G & \textsf{dnf} & \textsf{dnf} & \textbf{2G} & 0.678 & 0.683 & \textsf{dnf} & \textsf{dnf} & 0.678 
		%		& \textsf{dnf} & \textbf{0.1}
		\\
		& & Twitter & 41.7\textsf{M} & 1.5\textsf{B} & \textsf{mem} & \textsf{mem} & \textsf{dnf} & \textsf{dnf} & \textbf{1.6h} & \textsf{mem} & \textsf{mem} & \textsf{dnf} & \textsf{dnf} &  \textbf{18G} & \textsf{mem} & \textsf{mem} & \textsf{dnf} & \textsf{dnf} & 0.243
		%		& \textsf{dnf} & \textbf{0.9} 
		\\	
		& & Friendster & 65.6\textsf{M} & 3.6\textsf{B} & \textsf{mem} & \textsf{mem} & \textsf{dnf} & \textsf{dnf} & \textbf{11.2h} & \textsf{mem} & \textsf{mem} & \textsf{dnf} & \textsf{dnf} & \textbf{35G} & \textsf{mem} & \textsf{mem} & \textsf{dnf} & \textsf{dnf} & 0.396 
		%		& \textsf{dnf}  & \textbf{0.3} 
		\\ 
		\midrule
		\multirow{6}{*}{\textsf{WC}} & \multirow{3}{*}{\textsf{Small}}
		& PHY & 37 \textsf{K} & 181\textsf{K} & 10.1 & 0.7 & 4.2 & 0.6 & \textbf{0.5} & 285 & 369 & 170 & 52 & \textbf{18} & 0.068 & 0.056 & 0.068 & 0.067 & 0.066
		%		& 370.1 & \textbf{30.4}
		\\
		& & Epinions & 132\textsf{K} & 841\textsf{K} & 32.8 & 0.5 & 7.6 & 0.7 & \textbf{0.2} & 568 & 399 & 115 & 42 & \textbf{25} & 0.196 & 0.151 & 0.196 & 0.195 & 0.184 
		%		& 123.0 & \textbf{2.7} 
		\\
		& & DBLP & 655\textsf{K} & 2\textsf{M} & 399.7 & 4.2 & 12.6 & 0.8 & \textbf{0.5} & 5G & 949 & 331 & 151 & \textbf{137} & 0.109 & 0.090 & 0.109 & 0.108 & 0.105 
		%		& 3171.0 & \textbf{172.2}
		\\
		\cmidrule{3-20}
		& \multirow{3}{*}{\textsf{Large}}
		& Orkut & 3\textsf{M} & 234\textsf{M} & 3.2h & \textbf{14.4} & 0.4h & 80.1 & 21.8 & 28G & 8G & 6G & \textbf{2G} & \textbf{2G} & 0.067 & 0.060 & 0.067 & 0.066 & 0.064
		%		& \textsf{dnf} & \textbf{0.1}
		\\
		& & Twitter & 41.7\textsf{M} & 1.5\textsf{B} & \textsf{dnf} & \textsf{mem} & 1.6h & 102.7 & \textbf{14.91} & \textsf{dnf} & \textsf{mem} & 30G & \textbf{16G} & \textbf{16G} & \textsf{dnf} & \textsf{mem} & 0.259 & 0.257 & 0.247
		%		& \textsf{dnf} & \textbf{0.9} 
		\\	
		& & Friendster & 65.6\textsf{M} & 3.6\textsf{B} & \textsf{dnf} & \textsf{mem} & \textsf{mem} & 3.3h & \textbf{0.9h} & \textsf{dnf} & \textsf{mem} & \textsf{mem} & \textbf{43G} & 47G & \textsf{dnf} & \textsf{mem} & \textsf{mem} & 0.004 & 0.004
		\\
		\bottomrule    		
	\end{tabularx}
	\label{tab:compare_im}
	\vspace{-0.15in}
\end{table*}
\begin{figure*}[!ht] \centering
	\includegraphics[width=0.4\linewidth]{figures/legend}
	\vspace{-0.25in}
\end{figure*}
\begin{figure*}[!ht]
	\vspace{-0.1in}
	\subfloat[Epinions (\textsf{TRI})]{
		\includegraphics[width=0.24\linewidth]{figures/epinions_IC_trivalency_time}
		%		\label{fig:hep_lt_inf}
	}
	\subfloat[Orkut (\textsf{TRI})]{
		\includegraphics[width=0.24\linewidth]{figures/dblp_IC_trivalency_time}
		%		\label{fig:phy_lt_inf}
	}
	\subfloat[Epinions (\textsf{WC})]{
		\includegraphics[width=0.24\linewidth]{figures/epinions_IC_d1_time}
		%		\label{fig:hep_lt_inf}
	}
	\subfloat[Orkut (\textsf{WC})]{
		\includegraphics[width=0.24\linewidth]{figures/dblp_IC_e1_time}
		%		\label{fig:phy_lt_inf}
	}
	\vspace{-0.1in}
	\caption{Running time across different $k$ on \textsf{TRI} and \textsf{WC} models.}
	\label{fig:time_ic}
	\vspace{-0.15in}
\end{figure*}
\begin{figure*}[!ht] \centering
	\includegraphics[width=0.4\linewidth]{figures/legend}
	\vspace{-0.35in}
\end{figure*}
\begin{figure*}[!ht]
	\subfloat[Epinions (\textsf{TRI})]{
		\includegraphics[width=0.24\linewidth]{figures/epinions_IC_trivalency_mem}
		%		\label{fig:hep_lt_inf}
	}
	\subfloat[Orkut (\textsf{TRI})]{
		\includegraphics[width=0.24\linewidth]{figures/dblp_IC_trivalency_mem}
		%		\label{fig:phy_lt_inf}
	}
	\subfloat[Epinions (\textsf{WC})]{
		\includegraphics[width=0.24\linewidth]{figures/epinions_IC_e1_mem}
		%		\label{fig:hep_lt_inf}
	}
	\subfloat[Orkut (\textsf{WC})]{
		\includegraphics[width=0.24\linewidth]{figures/dblp_IC_e1_mem}
		%		\label{fig:phy_lt_inf}
	}
	\vspace{-0.1in}
	\caption{Memory usage across different $k$ on \textsf{TRI} and \textsf{WC} models.}
	\label{fig:mem_ic}
	\vspace{-0.2in}
\end{figure*}

%\subsubsection{Experimental Settings}

%\setlength\tabcolsep{4pt}
%\begin{table}[!h]
%%	\vspace{-0.1in}
%	\caption{Centrality Maximization Datasets}
%	\vspace{-0.1in}
%	\label{tab:data_sum_s}
%	\centering
%	\begin{tabular}{ l  r  r  r }\toprule	
%		\textbf{Dataset} & \bf \#Nodes& \bf \#Edges & \bf Avg. degree\\\midrule
%		Ego-Facebook & 4 K & 88 K & 43.7 \\
%		CA-GrQc & 5 K & 14 K & 5.6 \\
%		CA-HepTh & 10 K & 26 K & 5.3 \\
%		Email-Enron & 37 K & 184 K & 10.0 \\
%		%		p2p-Gnutella08 & 6301 & 20777 & 6.6 \\
%		loc-Brightkite & 58 K & 214 K & 7.4 \\
%		soc-Epinions1 & 76 K & 509 K & 10.7\\
%		\bottomrule
%	\end{tabular}
%%	\vspace{-0.1in}
%\end{table}

%\textbf{Datasets.} Since \exhaust{} cannot run on large networks, we use six moderate-sized network datasets described in Table~\ref{tab:compare_bcm} which have been widely used in previous studies \cite{Mahmoody16,Yoshida14}.

\vspace{0.03in}

\noindent \textbf{Running time.}
Table~\ref{tab:rtime} presents the running time of \dta{} and five existing algorithms on four centrality maximization problems. The results show that \dta{} runs much faster than other algorithms,i.e. the speedup is in orders of magnitude. Specifically, compared to the second fastest algorithm - the adaptations of \DPIMA{}, \dta{} maintains a good gap of 10-20 times faster. Compared to other approaches, \dta{} shows much more significant speedup of $>$100x faster. This observation is seen clearly on betweenness and coverage maximizations since the sampling are very expensive.

\vspace{0.03in}

\noindent \textbf{Memory.}
Table~\ref{tab:mem_relative} presents the average relative memory of different algorithms to that of \dta{}, i.e. their memory usage divided by \dta{}'s. \dta{} uses several times less memory than others. \hedge{} and \yalg{} uses similar memory since they follow the same heuristic setting on the number of samples.

\vspace{0.03in}

\noindent \textbf{Solution quality.}
The quality of solution returned by different algorithms is presented in Table~\ref{tab:qual_relative}. We observe that all the algorithms provide similar solution quality. 
%An interesting pattern combining Tables~\ref{tab:qual} and \ref{tab:sample} is that the solution quality of \dta{} is highly correlated with the number of samples needed. Specifically, it needs more samples if the solution has lower quality in the network. For example, on \BCM{}, \dta{} needs only 211 samples on Ego-Facebook but requires over 5000 samples on CA-HepTh because the solution on Ego-Facebook has quality of 0.92 while on CA-HepTh, it is only 0.51. This correlation is not observed on other algorithms which require more samples for larger networks.

%\subsection{Landmark selection on large networks}
%\setlength\tabcolsep{2pt}
%\begin{table}\small
%	\centering
%	\caption{Running time and memory usage of landmark selection algorithms on large-scale networks.}
%	\vspace{-0.1in}
%	\begin{tabular}{l rrr rrr }
%		\toprule
%		&  \multicolumn{3}{c}{\textbf{Running time (s)}} & \multicolumn{3}{c}{\textbf{Memory usage (MB)}} \\
%		\cmidrule(lr){2-4} \cmidrule(lr){5-7} 
%		\textbf{Data} & \IMM$_c$ & \SSA$_c$ & \dta{} & \IMM$_c$ & \SSA$_c$ & \dta{} \\
%		\midrule
%		PHY &  \\
%		Epinions &  \\
%		DBLP &  \\
%		Orkut & \\
%		Twitter &  \\
%		\bottomrule
%	\end{tabular}
%	\label{tab:landmark}
%\end{table}

%\subsubsection{Betweenness Centrality Maximization}
%Table~\ref{tab:compare_bcm} shows the running time, memory usage, and achieved betweenness centrality of four algorithms for the \BCM{} problem with $k=100$. Compared to the most recent methods, i.e. \hedge{} and \yalg{}, we observe that \dta{} runs 30 times faster than the second place \yalg{} while the speedup factor is 70x over the most recent \hedge{}. In terms of memory usage, \dta{} also uses several times less memory than the others. Af course, all three approximation algorithms, i.e. \dta{}, \hedge{} and \yalg{}, run dramatically faster than \exhaust{}. \exhaust{} fails to run on the last two largest datasets due to requiring more than 12h to finish.

%Interestingly, combined these speedups and memory savings with the number of samples acquired, \dta{} uses more samples than both \hedge{} and \yalg{} but still consumes much less time and memory. This exhibits the power of steadily building up the solution $S$ on the fly and threshold $z$ in \dta{} algorithm. Since, a partial solution $S$ is known, $S$ is immediately used to early terminate sample generation as soon as a node in $S$ appears to save time. 
%That sample is eliminated with updates on $d_S$ to save memory. 
%Note that, although \hedge{} and \yalg{} algorithm use a small number of samples, they fail to deliver approximation guarantees.
% to the returned solution while \dta{} does.

%Comparing the obtained betweenness centralities of returned solutions, the two algorithms, i.e. \dta{}, \yalg{} achieve similar level of solution quality which is most of the times higher than that of \hedge{}. \exhaust{} always maintains a gap to other algorithms.

%\subsubsection{Coverage, Motif-based and $K$-path Centrality Maximizations}
%Tables~\ref{tab:compare_ccm} and~\ref{tab:compare_triangle} give the results of algorithms on coverage, triangle and $K$-Path centrality maximization problems\footnote{\hedge{} algorithm \cite{Mahmoody16} works on both coverage and triangle problems, however, the implementation obtained from the authors did not support these features yet.}. Similar observations seen in \BCM{} experimental results are observed for both coverage and triangle and $K$-Path centrality maximization. \dta{} runs considerably faster and consumes less memory than other algorithms. Notice that in these problems, \dta{} seems to achieve better quality than \yalg{} and get closer to \exhaust{}.
%Notably, the quality of \dta{} most of the times surpass \yalg{} on \CCM{} and \exhaust{} algorithm for triangle centrality maximization is relatively fast.

%\subsubsection{$K$-path centrality maximization}

\subsection{Results on Influence Maximization}

%Thus, we present our comparison results between \dta{} and these two main algorithms. Extended experiments on other algorithms, including the recent \DPIMA{} algorithm \cite{Nguyen163} that was shown to outperform the other \IM{} algorithms but contains technical errors, can be found in \cite{extend}.
% The authors publish technical report in \cite{dssafixed} that seems to fix the errors but have not gone through peer-reviewed. Thus, we include comparison between our algorithm and other algorithms including \DPIMA{} in our extended version in \cite{extend}.
%Since we have two upper-bound functions: the requirement and the top-$k$, we call the \dta{} algorithm combined with each of these functions \dta-\textsf{req} and \dta-\textsf{top} respectively.
%
%\setlength\tabcolsep{4pt}
%\begin{table}[!htb]
%%	\vspace{-0.1in}
%	\caption{\IM{} Datasets}
%	\vspace{-0.1in}
%	\label{tab:data_sum}
%	\centering
%	\begin{tabular}{l r r r}
%		\toprule	
%		\textbf{Dataset} & \bf \#Nodes& \bf \#Edges & \bf Avg. degree\\
%		\midrule
%		PHY\footnotemark[\value{footnote}] & 37 K & 181 K & 13.4\\
%		Epinions\footnotemark[\value{footnote}] & 132 K & 841 K & 13.4\\
%		DBLP\footnotemark[\value{footnote}] & 655 K & 2 M & 6.1\\
%		Orkut\footnotemark[\value{footnote}] & 3 M & 234 M & 78\\
%		Twitter \cite{Kwak10} & 41.7 M & 1.5 B & 70.5\\
%		Friendster\footnotemark[\value{footnote}] & 65.6 M & 3.6 B & 54.8\\
%		\bottomrule
%	\end{tabular}
%%	\vspace{-0.1in}
%\end{table}
\textbf{Model Settings.}
For computing edge weights, we consider the widely-used \textit{Trivalency} (\textsf{TRI}) model \cite{Cohen14, Chen10, Jung12} which selects the weight of $w(u,v)$ randomly from the set of influence probabilities $\{0.1, 0.01, 0.001\}$, and \textit{Weighted Cascade }(\textsf{WC})  model \cite{Chen09_2,Tang14,Tang15,Nguyen163} that sets the weight of $(u,v)$ disproportional to in-degree of $v$, i.e. $w(u,v) = 1/d_{in} (v)$.

We consider the Independent Cascade (\textsf{IC}) \cite{Domingos01,Kempe03} for diffusion modeling. To verify the quality of a solution, we adopt the approach in \cite{Nguyen172} that provides estimation within $\epsilon=0.01$ error from the true influence with prob. $1/n$.
%	\item \textit{Weighted Cascade} (\textsf{WC}) \cite{Tang14,Cohen14,Tang15,Nguyen163}: The weight of edge $(u,v)$ is inversely proportional to the in-degree of node $v$, $d_{in}(v)$, i.e. $w(u,v) = \frac{1}{d_{in}(v)}$.
%\end{itemize}

%\textbf{Algorithms' parameter settings.} For our algorithm and \IMM{}, we set the $\epsilon=0.5$ that controls the solution quality. For \PMC{}, we take the recommended parameter of 200 DAGs.

%\subsubsection{Comparison of \dta{} with other \IM{} algorithms}
%<<<<<<< HEAD
%The experimental results in terms of running time, memory usage, solution quality and the number of \RIS{} samples are presented in Table~\ref{tab:compare_im}.
%
%All the results consistently show that \dta{} algorithm achieves significantly better performance than other existing algorithms, i.e. running 40x faster and using 15x less memory than the runner-up. These huge time and memory savings prove the effectiveness of our thresholding strategy and tightness of the empirical error bounding techniques. As a result, \dta{} algorithm is the only one that can run on the largest billion-edge Twitter and Friendster networks.
%=======

\vspace{0.03in}

\noindent \textbf{Results Overview.} The experimental results in terms of running time, memory usage, solution quality are presented in Table~\ref{tab:compare_im} and Figures~\ref{fig:time_ic} and \ref{fig:mem_ic}. The results consistently show that \dta{} algorithm achieves significantly better running time and memory usage, i.e. orders of magnitudes faster and using at least 15x less memory. Our observations are consistent with the recent benchmark in \cite{Arora17} that most existing \IM{} methods do not scale well on the \textsf{TRI} model.
%These huge time and memory savings prove the effectiveness of our thresholding strategy and tightness of the empirical error bounding techniques. As a result, \dta{} algorithm is the only one that can run on the largest billion-edge Twitter and Friendster networks.

\vspace{0.03in}

\noindent \textbf{Running time.} From Table~\ref{tab:compare_im}, we see that \dta{} significantly outpaces the other algorithms. \dta{} always maintains large gaps to other algorithms on both models, e.g. up to 20x faster than \DPIMA{} and 100x faster than \IMM{}. \dta{} is the only algorithm that can run on Twitter and Friendster for the challenging \textsf{TRI} model while \DPIMA{} and \IMM{} fail on all large networks. \textsf{TipTop} cannot run on the last two largest networks on both \textsf{WC} and \textsf{TRI}. \PMC{} seems to handle \textsf{TRI} model week but struggles on \textsf{WC}.
%\textbf{Compare running time.} From Table~\ref{tab:compare_im}, we see that \dta{} completely outpaces the other algorithms. \dta{} always maintains large gaps to other algorithms, e.g. up to 40x and 100x respectively faster than \DPIMA{} and \IMM{} which provide the same approximation guarantees as \dta{}. \IMM{} fails even on Orkut and \DPIMA{} cannot run for the largest two networks. In contrast, \dta{} algorithm needs less than half of hour on Twitter and 2.3 hours on the biggest Friendster.
%An interesting observation is that \textsf{PMC} works relatively well on \textsf{TRI} model but experiencing much difficulty on the \textsf{WC} model, while \IMM{} and \DPIMA{} show the inverse, i.e. performing better on \textsf{WC} than \textsf{TRI}.
%>>>>>>> 35e69f553eb13251a19506af3916f0e55b196828
%<<<<<<< HEAD
%<<<<<<< HEAD
%\textbf{Compare running time.} From Table~\ref{tab:compare_im}, we see that both versions of \dta{} algorithm, i.e. \dta-\textsf{req} and \dta-\textsf{top}, clearly show their advantages on the \textsf{TRI} model. \dta{} always maintains large gaps to other algorithms, e.g. up to 40x and 100x respectively faster than \DPIMA{} and \IMM{} which provide the same approximation guarantees as \dta{}. \IMM{} fail to run even on Orkut and \DPIMA{} cannot fun for the largest two networks. In contrast, \dta{} algorithm need less than half of hour on Twitter and 2.3 hours on the biggest Friendster.
%=======
%\textbf{Compare running time.} From Table~\ref{tab:compare_im}, we see that \dta{} completely outpaces the other algorithms. \dta{} always maintains large gaps to other algorithms, e.g. up to 40x and 100x respectively faster than \DPIMA{} and \IMM{} which provide the same approximation guarantees as \dta{}. \IMM{} fails even on Orkut and \DPIMA{} cannot run for the largest two networks. In contrast, \dta{} algorithm needs less than half of hour on Twitter and 2.3 hours on the biggest Friendster.
%>>>>>>> a5a344d958afcd6499f3a1c90a4daeae69551496
%%An interesting observation is that \textsf{PMC} works relatively well on \textsf{TRI} model but experiencing much difficulty on the \textsf{WC} model, while \IMM{} and \DPIMA{} show the inverse, i.e. performing better on \textsf{WC} than \textsf{TRI}.
%
%=======
%>>>>>>> 35e69f553eb13251a19506af3916f0e55b196828
Results over a wide range of $k$ in Figure~\ref{fig:time_ic} show similar observations.

\vspace{0.03in}

\noindent \textbf{Memory.} The observations on running time hold on memory comparison. \dta{} algorithm consumes much less memory than the rest. Notably, on the large Orkut network with 234 million edges, \dta{} only uses 2GB while \PMC{} requires 21GB - 10.5 times more memory than \dta{} consumption and \textsf{TipTop} uses 89GB - 44.5x greater than that of \dta{}. They fail to run on larger networks due to running out of 100GB. On \textsf{WC} model, \dta{} and \DPIMA{} use similar amount of memory and are the only algorithms that can run on all the networks on this model. Similar observations are seen from Figure~\ref{fig:mem_ic} on different value of $k$.
%\PMC{} seems to work better than \DPIMA{} and \IMM{} on the \textsf{TRI} edge model, however, this is only true on networks of small sizes. 
%\PMC{} fails to run on both Twitter and Friendster due to excessive memory requirement. On the other hand, \dta{} requires the maximum of 37GB on the largest Friendster leaving plenty of room for running much larger networks.

%We also tried to run the runner-up \DPIMA{} algorithm till finish allowing more memory and time and observe that \DPIMA{} requires 109GB in 12.6 hours while \dta{} only needs 16GB in 2.3 hours.

%\setlength\tabcolsep{2pt}
%\begin{table}[!h] \small
%	\centering
%	\caption{Coverage Centrality Maximization (\CCM{}) problem for $k=100$. }
%	\vspace{-0.15in}
%	\begin{tabular}{l rrr r rrr r rrr r rr}
%		\toprule
%		& \multicolumn{3}{c}{\textbf{Time [s (or h)]}} && \multicolumn{3}{c}{\textbf{Memory [M (or G)]}} && \multicolumn{3}{c}{\textbf{Coverage}} && \multicolumn{2}{c}{\textbf{\#Samples }} \\
%		\cmidrule{2-4}  \cmidrule{6-8} \cmidrule{10-12} \cmidrule{14-15} 
%		\textbf{Data} & \exhaust{} & \yalg{} & \dta{}  && \exhaust{} & \yalg{} & \dta{}  && \exhaust{} & \yalg{} & \dta{}  && \yalg{} & \dta{} \\
%		\midrule			
%		Ego-F. & 525.1 & 0.1 & \textbf{0.0} && 13.5 & 14.5 & \textbf{5.0} && 0.99 & 0.97 & 0.94 && 205 & 498 \\
%		CA-G. & 670.8 & \textbf{0.0} & \textbf{0.0} && 12.7 & 13.1 & \textbf{3.2} && 0.60 & 0.39 & 0.50 && 212 & 919 \\
%		CA-H. & 0.9h & 0.1 & \textbf{0.0} && 13.4 & 13.4 & \textbf{4.30} && 0.65 & 0.39 & 0.50 && 227 & 872 \\
%		Email & 14.8h & 0.6 & \textbf{0.1} && 17.0 & 18.6 & \textbf{13.6} && 0.82 & 0.65 & 0.70 && 258 & 824 \\
%		loc-B. & \textsf{dnf} & 1.2 & \textbf{0.1} &&\textsf{dnf}& 20.4 & \textbf{18.4} &&\textsf{dnf}& 0.74 &0.76 && 269 & 777 \\
%		soc-E. & \textsf{dnf} & 2.1 & \textbf{0.2} &&\textsf{dnf}& \textbf{22.7} & 24.1 &&\textsf{dnf}& 0.72 & 0.76 && 276 & 789\\
%		\bottomrule    		
%	\end{tabular}
%	\label{tab:compare_ccm}
%	\vspace{-0.1in}
%\end{table}

\vspace{0.03in}

\noindent \textbf{Solution quality.} 
Results from Table~\ref{tab:compare_im} show that most algorithms provide similar solution quality except \textsf{TipTop}. This is due to that \textsf{TipTop} uses stochastic programming to find exact solution on the generated samples, thus, \textsf{TipTop} can find solution almost matching the approximation ratio.
%shows solution quality results for the tested algorithms and reveals that for $\epsilon = 0.5$, \dta{} returns worse quality than \IMM{} and \PMC{}. This is due to the fact that \dta{} is able to detect precisely the moment that the required $(1-1/e-\epsilon)$-guarantee is attained while \IMM{} and \PMC{} fail to do so (clearly shown in the next experiments with multiple $\epsilon$ values). Moreover, both \dta{} and \IMM{} rely on \RIS{} sampling and more \RIS{} samples provide better solution quality. We observe that \dta{} needs considerably fewer samples than \IMM{}.
%Here we test the second versions of \dta{} algorithm, denoted by $\rho$\dta{}-\textsf{req} and $\rho$\dta{}-\textsf{top}, taking into account the empirical approximation ratio of the \tpa{} component in \dta{} algorithm. By Lemma~\ref{lem:anyz}, the solution $S_z$ found by \tpa{} satisfies $\Cov^{(T)}(S_z) \geq \rho_k z \geq (1-1/e)\OPT_k$. Hence, $\frac{\Cov^{(T)}(S_z)}{z} \geq (1-1/e)$ is a better empirical approximation quality of $S_z$. In new versions, we replace the stopping condition in Line~4, i.e. $\rho_z \geq 1-1/e-\epsilon$, by $\rho_z \geq \frac{\Cov^{(T)}(S_z)}{z} - \epsilon$. Note that both $\rho$\dta{}-\textsf{req} and $\rho$\dta{}-\textsf{top} still maintain the worst case guarantee of $(1-1/e-\epsilon)$ w.h.p. The reasons for this consideration are two-fold: 1) use a better empirical bound; 2) improve the solution quality since the ratio is within $\epsilon$ of the actual observed $\frac{\Cov^{(T)}(S_z)}{z}$. 
%Clearly, the high quality version $\tpa_{hq}$ performs better than \dta{} due to better bounds.

%From Figure~\ref{fig:inf}, another observation is that the \dta{} algorithm with the \textsf{top}-$k$ function perform better than those with the requirement. This is attributed to the fact that \textsf{top}-$k$ function finds a better bound and, thus, the \tpa{} component obtains a higher quality solution. Furthermore, we see that all the algorithms return solutions with quality better than the worst-case bound of $(1-1/e-\epsilon)$.
%
%\textbf{Compare \#Samples.} \dta{} algorithm also have minimal sample requirement compared to the others. They use at least 20 times fewer samples than that of \IMM{}.
% This pattern holds on both \textsf{TRI} and \textsf{WC} models.

%\subsubsection{Comparison of upper-bound functions on \dta{} algorithm}
%We next compare the two upper-bound functions that are used in \dta{} algorithm: the requirement and top-$k$ functions. We run two version of \dta{} using those upper-bound functions on all the datasets and compute the relative ratios of influences obtained by the two versions and their running times:
%\begin{align}
%	\frac{\I(S_{\dta-\textsf{top}})}{\I(S_{\dta-\textsf{req}})} \cdot 100 \text{ } and \text{  } \frac{\textsf{Time}(\dta-\textsf{top})}{\textsf{Time}(\dta-\textsf{req})} \cdot 100.
%\end{align}
%The  averages of obtained influences and times over all the networks are shown in Figure~\ref{fig:bounds}. The results show a noticeable improvement in terms of solution quality when the stronger top-$k$ upper-bound function is used compared to that of the basic requirement function. This improvement can go up to 10\% on the \textsf{WC} model and 5\% on \textsf{TRI} for $k$ between 100 and 5000. However, the increase of running time when top-$k$ function applies is very striking. This phenomenon is due to the fact that top-$k$ bound is tighter than the requirement bound, that may cause \dta{} to acquire more samples to reach the threshold $z$. This increases of running time appears everywhere on \textsf{TRI} model while it only happens for $k=1$ under the \textsf{WC}.

%\subsubsection{Parallel \dta{} implementation}

%\setlength\tabcolsep{2pt}
%\begin{table}[!h] \small
%	\centering
%	\caption{Motif-based Centrality Maximization. }
%	\vspace{-0.15in}
%	\begin{tabular}{l rr r rr}
%		\toprule
%		& \multicolumn{2}{c}{\textbf{Running Time [s (or h)]}} && \multicolumn{2}{c}{\textbf{Total Memory [M (or G)]}} \\
%		\cmidrule{2-3}  \cmidrule{5-6}
%		\textbf{Data} & \exhaust{} & \dta{}  && \exhaust{} & \dta{} \\
%		\midrule			
%		Ego-Facebook & 0.1 & \textbf{0.0} & 15.5 & \textbf{10.0} \\
%		CA-GrQc & \textbf{0.0} & \textbf{0.0} & 13.3 & \textbf{8.5} \\
%		CA-HepTh & \textbf{0.0} & \textbf{0.0} & 14.1 & \textbf{10.3} \\
%		Email-Enron & 0.2 & \textbf{0.0} & 22.3 & \textbf{17.8} \\
%		loc-Brightkite & 0.1 & \textbf{0.0} & 25.3 & \textbf{22.5} \\
%		soc-Epinions1 & 0.2 & \textbf{0.0} & 29.1 & \textbf{28} \\
%		\bottomrule    		
%	\end{tabular}
%	\label{tab:compare_motif}
%	\vspace{-0.15in}
%\end{table}

\subsection{Time/Space-quality Trade-off}
\begin{figure}[!ht]
	\vspace{-0.65in}
	\includegraphics[width=1\linewidth]{figures/epsilon_tri_2}
	\vspace{-0.85in}
	\caption{\IM{} experiments on different desired approximation ratio on DBLP network and \textsf{TRI} edge-weight model.}
	\label{fig:inf}
	\vspace{-0.05in}
\end{figure}
%\renewcommand{\arraystretch}{0.9}
%\setlength\tabcolsep{3pt}
%\begin{table*}[!h] \small
%	\centering
%	\vspace{-0.05in}
%	\caption{Comparison of different upper-bound functions of \dta{} and \tpa{} for $k = 100$ and $\epsilon = 0.1$ on ego-Facebook network.}
%	\vspace{-0.1in}
%	\begin{tabularx}{\textwidth}{c *{18}{Y}}
%		\toprule
%		& \multicolumn{6}{c}{\textbf{Time [s (or h for hour)]}} & \multicolumn{6}{c}{\textbf{Memory [MB (or G for GB)]}} & \multicolumn{6}{c}{\textbf{Quality}} \\
%		\cmidrule(lr){2-7} \cmidrule(lr){8-13} \cmidrule(l){14-19}
%		Problem & \dta{} (\textsf{req}) & \dta{} (\textsf{top}) & \dta{} (\textsf{df2d}) & \tpa{} (\textsf{req}) & \tpa{} (\textsf{top}) & \tpa{} (\textsf{df2d}) & \dta{} (\textsf{req}) & \dta{} (\textsf{top}) & \dta{} (\textsf{df2d}) & \tpa{} (\textsf{req}) & \tpa{} (\textsf{top}) & \tpa{} (\textsf{df2d}) & \dta{} (\textsf{req}) & \dta{} (\textsf{top}) & \dta{} (\textsf{df2d}) & \tpa{} (\textsf{req}) & \tpa{} (\textsf{top}) & \tpa{} (\textsf{df2d}) \\
%		\midrule
%		\BCM{} & 0.02 & 0.02 & 0.03 & 38.40 & 39.03 & 52.89 & 6.34 & 6.34 & 6.37 & 8.77 & 21.79 & 8.78 & 0.92 & 0.91 & 0.92 & 0.96 & 0.96 & 0.96 \\
%		\CCM{} & 0.03 & 0.03 & 0.04 & 51.15 & 50.68 & 67.65 & 6.35 & 6.32 & 6.37 & 8.53 & 18.85 & 8.30 & 0.97 & 0.97 & 0.97 & 0.99 & 0.99 & 0.99 \\
%		\TCM{} & 0.05 & 0.03 & 0.09 & 1.20 & 1.36 & 2.29 & 7.72 & 9.27 & 7.48 & 42.20 & 47.97 & 44.36 & 0.21 & 0.20 & 0.19 & 0.19 & 0.19 & 0.19 \\
%		\PCM{} & 0.04 & 0.02 & 0.03 & 1.84 & 2.46 & 23.67 & 8.82 & 8.36 & 8.12 & 134.41 & 172.77 & 324.57 & 0.17 & 0.16 & 0.15 & 0.18 & 0.18 & 0.18 \\
%		\IM{} & 0.03 & 0.02 & 0.16 & 2.29 & 2.59 & 9.18 & 8.04 & 4.90 & 8.05 & 90.32 & 103.88 & 89.52 & 0.25 & 0.23 & 0.24 & 0.26 & 0.26 & 0.26 \\
%		
%		%		\midrule
%		%		\BCM{} & 0.65 & 0.41 & 0.94 & 160.89 & 176.37 & 1010.96 & 29.18 & 29.19 & 29.47 & 74.78 & 99.79 & 111.07 & 0.63 & 0.61 & 0.62 & 0.67 & 0.67 & 0.67 \\
%		%		\CCM{} & 0.15 & 0.16 & 0.56 & 214.00 & 219.83 & 554.13 & 24.56 & 24.59 & 25.16 & 59.22 & 93.93 & 59.52 & 0.74 & 0.73 & 0.75 & 0.89 & 0.89 & 0.89 \\
%		%		\TCM{} & 0.20 & 0.18 & 1.26 & 15.09 & 16.79 & 114.46 & 24.00 & 24.00 & 24.62 & 80.07 & 94.07 & 86.01 & 0.23 & 0.26 & 0.24 & 0.28 & 0.28 & 0.26 \\
%		%		\PCM{} & 0.07 & 0.02 & 0.47 & 5.30 & 7.47 & 538.78 & 30.79 & 27.27 & 27.64 & 342.86 & 477.22 & 886.43 & 0.11 & 0.10 & 0.10 & 0.11 & 0.11 & 0.11 \\
%		%		\IM{} & 0.03 & 0.02 & 0.16 & 2.29 & 2.59 & 9.18 & 8.04 & 4.90 & 8.05 & 90.32 & 103.88 & 89.52 & 993.20 & 941.09 & 986.23 & 1048.85 & 1048.27 & 1048.06 \\
%		\bottomrule    		
%	\end{tabularx}
%	\label{tab:compare_bounds}
%	\vspace{-0.1in}
%\end{table*}

%\renewcommand{\arraystretch}{0.9}
%\setlength\tabcolsep{3pt}
%\begin{table}[!h] \small
%	\centering
%	\vspace{-0.05in}
%	\caption{Instance-specific bounds using different upper-bound function for solutions of \IM{} algorithms on PHY.}
%	\centering
%	\begin{tabular}{llrrrrr}
%		\toprule
%		\textbf{UB} & \textbf{\dta{}} & \textbf{\DPIMA{}} & \textbf{\IMM{}} & \textbf{\PMC{}} & \textbf{\textsf{TipTop}} & \textbf{Ave. time (s)}\\
%		\midrule
%		\textsf{Req.} & 0.45 & 0.46 & 0.42 & 0.48 & 0.38 & 0.64\\
%		\textsf{Top-$k$} & 0.51 & 0.53 & 0.53 & 0.54 & 0.46 & 0.65 \\
%		\textsf{DF-2D} & 0.45 & 0.47 & 0.49 & 0.49 & 0.39 & 0.66 \\
%		\textsf{DF} & 0.75 & 0.76 & 0.76 & 0.77 & 0.69 & 1.92 \\
%		\textsf{LP} & 0.77 & 0.81 & 0.79 & 0.80 & 0.70 & 151.38 \\
%		\textsf{ILP} & 0.79 & 0.82 & 0.82 & 0.80 & 0.71 & 382.88 \\
%		\bottomrule
%	\end{tabular}
%	\label{tab:quality_assess}
%\end{table}
It would be unrealistic to expect \dta{} algorithm to be faster, more memory efficient, and having better (empirical) solution quality at the same time. After all, \dta{} and its competitors, e.g., \TIM/\TIM+, \IMM, \SSA/\DPIMA{}, are all sample optimization algorithms. That is the more  samples they acquire, the better (empirical) solution quality they provide. The fair way to compare them is to measure their time/memory needed to provide the same theoretical solution guarantee, i.e., $(1-1/e -\epsilon)$. The less time and space one needs to deliver a given theoretical guarantee the better. In other words, the better solution guarantee one algorithm can provide for a fixed number of samples, the better the algorithm. In that sense, for example, IMM is better than TIM/TIM+, and our experiments indicate that \dta{} is better than all existing algorithms. 


We run different \IM{} algorithms with various approximation guarantees and compare the resulted expected influence, running time and memory usage.
% to an upper-bound of the optimal solution. Recall that $z$ in \tpa{} is a bound on the optimal coverage. Thus, $\frac{z}{T}n$ is an upper-bound of the estimate of optimal influence. To provide a good bound, we run \dta{} with very small $\epsilon = 0.001$ and consider $\frac{z}{T}n$ as $\OPTk$.
The results on DBLP network, which is the largest network that all the algorithms can handle on \textsf{TRI} model, are given in Figure~\ref{fig:inf}. We observe a nice curve expressed by \dta{} and \textsf{TipTop}, that is almost parallel with the worst-case bound $1-1/e-\epsilon$ line. That nice curve suggests a good control of solution quality based on parameter settings. On the other hand, \dta{} uses much less memory and time than \textsf{TipTop}, implying that \dta{} has better trade-off between quality and time/space.
%This gives a fine-grained trade-off between desired quality and cost, or a nice control of the solution based on $\epsilon$ value. 
In contrast, \IMM{} and \PMC{} provide mostly the same solution quality for different guarantees. This suggests that the bounds on these algorithm are conservative.

%\begin{figure}[!ht]
%	\vspace{-0.35in}
%	\includegraphics[width=\linewidth]{figures/bound_phy}
%	\vspace{-0.85in}
%	\caption{Relative performance of \dta{} to \textsf{EXHAUST} greedy.}
%	\label{fig:sum_exps}
%%	\vspace{-0.1in}
%\end{figure}
%
%\subsection{Comparison with \textsf{EXHAUST} Greedy}
%Figure~\ref{fig:sum_exps} gives results of \dta{} with requirement upper-bound function ($\epsilon = 0.1$) in comparison with the offline \exhaust{} greedy algorithm \cite{Mahmoody16} which runs on the set of all hyperedges (samples). Since \exhaust{} algorithm for Influence Maximization and $K$-Path are not available due to exponential number of samples, we use the state-of-the-art \IMM{} \cite{Tang15} and its adaptation to $K$-path sampling to replace \exhaust{}. The results show that, in all the applications, \dta{} returns comparable solution quality, i.e. $> 90\%$ effectiveness, to the offline \exhaust{} which assumes the complete hypergraph while using very tiny fraction of time needed by \exhaust{} greedy.
%
%Further, the results show that \dta{} algorithm illustrate definite advantage for betweenness and closeness centrality maximizations where it is very expensive to both compute the exact values and generate samples, i.e. shortest paths. \dta{}-\textsf{req} only requires several percent of time used by \exhaust{} and for larger networks, this percentage sets even smaller.
\renewcommand{\arraystretch}{1}
\setlength\tabcolsep{5pt}
\begin{table}[!htb] \small
	%	\vspace{-0.1in}
	\caption{Approximation bounds provided by different upper-bound functions (Higher bound implies better).}
	\vspace{-0.05in}
	\label{tab:ubounds2}
	\centering
	\begin{tabular}{ l r r r r r r}
		\toprule	
		\textbf{Data} & \bf \textsf{Req.} & \bf \textsf{Top-$k$} & \bf\textsf{DF-2D} & \bf\textsf{DF} & \bf LP & $d_S$\\
		\midrule
		%		PHY & 7266 & 7002 & 6400 & 4642 & 4504 & 4466 & 99.2\% \\
		%		Epinions & 1817 & 1817 & 1600 & 1592 & 1520 & 1517 & 99.8\% \\
		%		DBLP & 7428 & 7170 & 6400 & 4596 & 4537 & 4528 & 99.8\% \\
		%		Orkut & 498 & 446 & 400 & 400 & 400 & 400 & 100\%\\
		%		Twitter & 299& 299 & 200 & 200 & \textsf{dnf} & 200 & 100\%\\
		%		Friendster & 100 & 100 & 100 & 100 & \textsf{dnf} & 100 & 100\%\\
		PHY & 61.5\% & 63.8\% & 69.8\% & 96.2\% & 99.2\% & 4466  \\
		Epinions & 83.5\% & 83.5\% & 94.8\% & 95.3\% & 99.8\% & 1517  \\
		DBLP & 60.1\% & 63.2\% & 70.8\% & 96.5\% & 99.8\% & 4528 \\
		Orkut & 80.3\% & 89.7\% & 100\% & 100\% & 100\% & 400\\
		Twitter & 66.9\% & 66.9\% & 100\% & 100\% & \textsf{dnf} & 200 \\
		Friendster & 100\% & 100\% & 100\% & 100\% & \textsf{dnf} & 100\\
		\bottomrule
	\end{tabular}
	\vspace{-0.05in}
\end{table}
\renewcommand{\arraystretch}{0.9}
\setlength\tabcolsep{1.5pt}
\begin{table}[!h] \small
	\centering
%	\vspace{-0.05in}
	\caption{Performance of \dta{} and \tpa{} with different upper-bound (UB) functions on ego-Facebook.}
	\vspace{-0.1in}
	\centering
	\begin{tabular}{llrrrr}
		\toprule
		\textbf{Algo.} & \textbf{UB} & \textbf{Time (s)} & \textbf{Memory (MB)} & \textbf{Quality} & \textbf{\#Samples} \\
		\midrule
		\multirow{3}{*}{\dta{}} & \textsf{Req.} & 0.3 & 9.7 & 0.17 & 29.16x$10^3$ \\
		& \textsf{Top-$k$} & 0.2 & 8.4 & 0.16 & 16.68x$10^3$ \\
		& \textsf{DF-2D} & 0.4 & 8.8 & 0.16 & 6.38x$10^3$ \\
		\midrule
		\multirow{3}{*}{\tpa{}} & \textsf{Req.} & 1.8 & 135.2 & 0.18 & 2.11x$10^6$ \\
		& \textsf{Top-$k$} & 2.4 & 173.0 & 0.18 & 2.53x$10^6$ \\
		& \textsf{DF-2D} & 22.7 & 321.1 & 0.18 & 5.38x$10^6$ \\
		\bottomrule
	\end{tabular}
	\label{tab:compare_bounds}
\end{table}

\subsection{Comparison of Upper-bound Functions}
\textbf{Tightness of bounds.}
We compare the quality of the upper-bound functions, i.e. \textsf{Requirement}, \textsf{Top-$k$}, \textsf{LP}, \textsf{DF} and \textsf{DF-2D}, and use Influence Maximization to test. We run \dta{} algorithm ($\epsilon = 0.1$) with \textsf{DF-2D} upper-bound function to find a solution $S_k$ and compute the other upper-bounds on the same set of acquired hyperedges and $S_k$. The results are shown in Table~\ref{tab:ubounds2}.

From Table~\ref{tab:ubounds2}, on all datasets, we observe a clear order of upper-bound functions in terms of quality. The requirement function provides the worst bound while the \textsf{LP} has the tightest bound thanks to its optimality. 
%However, from Table~\ref{tab:ubound_fun}, this is also the increasing order of upper-bound functions in terms of complexity. Thus, better bound requires more computational resources. 
The \textsf{DF-2D} provides a reasonable bound with low complexity.

\vspace{0.03in}

\noindent \textbf{Effects of upper-bound function on \tpa{}, \dta{}.}
We run \dta{} and \tpa{} with three upper-bound functions that provide our favorable space bound of $\tilde{O}(\epsilon^{-2} n)$, i.e. \textsf{Requirement}, \textsf{Top-$k$} and \textsf{DF-2D}. The results on ego-Facebook are presented in Table~\ref{tab:compare_bounds}. It is clear that \dta{} runs much faster and uses much less memory than \tpa{} thanks to the tight empirical quality assessment. On the other hand, the tight assessment causes the solution quality of \dta{} to be slightly lower than that of \tpa{}. Compared between upper-bound functions, \textsf{Top-$k$} seems to use least time and memory but provides worst solution than \textsf{Requirement} and \textsf{DF-2D}. This may be attributed to the tighter bound provided by \textsf{Top-$k$}.

==> body/related.tex <==
\subsection{Related Work}

\textbf{Max-$k$-Cover.}
Max-$k$-Cover is a fundamental and core problem in extensive real-world applications ranging from circuit layout to designing marketing strategy (see \cite{Hochbaum96} and references therein for more applications). The problem is NP-hard \cite{Karp72} and the greedy algorithm \cite{Nemhauser81} that selects iteratively nodes with largest marginal gains gives the best achievable $(1-1/e)$-approximate solution \cite{Feige98}. The budgeted problem is studied in \cite{Khuller1999} where a tight $(1-1/e)$-approximate algorithm was proposed.

\textbf{Streaming Max-$k$-Cover.}
Algorithms for Max-$k$-Cover in different streaming data models have been studied in \cite{Mcgregor17,Bateni17,Saha09,Badanidiyuru14}. Notably, Saha and Getoor \cite{Saha09} gave an $\frac{1}{4}$-approximation algorithm using $\tilde{O}(km)$ space. \cite{Badanidiyuru14} proposed an $(\frac{1}{2}-\epsilon)$ approximation algorithm. Later, \cite{Mcgregor17,Bateni17} independently develop algorithms that achieve the best $(1-1/e-\epsilon)$ ratio for arbitrarily small $\epsilon$. Their algorithms only require a single pass and $\tilde{O}(\epsilon^3 n)$ and $\tilde{O}(\epsilon^2 n)$ memory space respectively. \cite{Mcgregor17,Saha09,Badanidiyuru14} study set-arrival model while \cite{Bateni17} focuses the edges arriving case.
%A comparison is given in Table~\ref{tab:algorithm}.


\textbf{Influence Maximization.}
Influence maximization (\IM{}) \cite{Domingos01,Leskovec07,Tang14,Tang15,Nguyen163,Goyal113,Chen2015,Li15,Lu15,Ohsaka16,Du13,Bakshy11} recently emerged from the vital application of designing a marketing strategy to maximize the benefit. Kempe et al. \cite{Kempe03} proved the submodularity property of influence function, thus, greedy algorithm provides an $(1-1/e-\epsilon)$-approximation guarantee. However, the naive greedy algorithm is not efficient due to the \#P-hardness of computing influences \cite{Chen10}. Lazy greedy technique was studied in \cite{Leskovec07}.
%Lazy greedy technique \cite{7} was investigated and shown to vastly improve the performance of naive greedy. 
Most recent algorithms based on \RIS{} sampling \cite{Borgs14} are summarized in Table~\ref{tab:algorithms}.
%Later, reverse influence sampling (\RIS) \cite{Borgs14} was introduced and \RIS{}-based algorithms \cite{Tang14,Tang15,Nguyen16,Nguyen163} were able to scale up to networks with millions of nodes and billions of edges. More practical applications of \IM{} were examined in \cite{Goyal113,Chen2015,Li15,Li152,Lu15,Ohsaka16,Du13}.

\textbf{Centrality Maximizations.}
Node centralities, e.g. Betweenness, Coverage, Triangle, $K$-path, etc. (see \cite{Easley10}) and their maximization problems have been widely studied in \cite{Yoshida14,Mahmoody16,Brandes07}. Most notable works on centrality maximization are shown in Table~\ref{tab:algorithms}.
%Notably, \cite{Yoshida14} proposed a sampling-based algorithm that generates $O(\epsilon^{-2}\log n)$ samples and guarantees an $((1-1/e)\OPTk - \epsilon n^{2})$-approximate solution for the betweenness and coverage centrality maximizations. More recently, Mahmoody et al. \cite{Mahmoody16} also relied on sampling technique and aimed to develop an $(1-1/e-\epsilon)$-approximation algorithm. However, the number of samples that provides the guarantees in \cite{Mahmoody16} depends on the unknown optimal solution and an heuristic replacement number $\epsilon^{-2} k \log n$ is utilized in their implementation. A summary of recent algorithms is provided in Table~\ref{tab:centrality}.

%\renewcommand{\arraystretch}{1}
%\setlength\tabcolsep{1.5pt}
%\begin{table}[!h]
%%	\vspace{-0.1in}
%	\caption{Summary of centrality maximization algorithms.}
%	\vspace{-0.15in}
%	\label{tab:centrality}
%	\centering
%	\begin{tabular}{cccc}
%		\toprule
%		Credit & Problems & Assumptions & Approx. \\
%		\midrule
%		\cite{Yoshida14} & \BCM{}, \CCM{} & none & $(1-\frac{1}{e})\OPTk - \epsilon n^2$ \\
%		\cite{Mahmoody16} & \BCM{}, \CCM{}, \TCM{}, \PCM{} & $\OPTk = \Omega(m)$ & $(1-\frac{1}{e}-\epsilon)$ \\
%		Here & \BCM{}, \CCM{}, \TCM{}, \PCM{} & none & $(1-\frac{1}{e}-\epsilon)$ \\
%		\bottomrule
%	\end{tabular}
%	\vspace{-0.1in}
%\end{table}

%Approximation bounds for centrality maximization problems



%\subsection{Network Interdiction}
%
%	\textbf{Triangle Interdiction}
%
%	\textbf{Epidemics Interdiction}


